Can the Utility of Anonymized Data be used for Privacy Breaches?

Group based anonymization is the most widely studied approach for privacy preserving data publishing. This includes k-anonymity, l-diversity, and t-closeness, to name a few. The goal of this paper is to raise a fundamental issue on the privacy exposure of the current group based approach. This has been overlooked in the past. The group based anonymization approach basically hides each individual record behind a group to preserve data privacy. If not properly anonymized, patterns can actually be derived from the published data and be used by the adversary to breach individual privacy. For example, from the medical records released, if patterns such as people from certain countries rarely suffer from some disease can be derived, then the information can be used to imply linkage of other people in an anonymized group with this disease with higher likelihood. We call the derived patterns from the published data the foreground knowledge. This is in contrast to the background knowledge that the adversary may obtain from other channels as studied in some previous work. Finally, we show by experiments that the attack is realistic in the privacy benchmark dataset under the traditional group based anonymization approach.

==> newton.tex <==


\if 0
It is noted that, in Example~\ref{example:exampleIllustrateGlobal},
implicitly, the equality $f_{11} + f_{12} = 1$ can be achieved.

\begin{lemma}
$f_{11} + f_{12} = 1$
\end{lemma}
\textbf{Proof:}
  \begin{eqnarray*}
     & & f_{11} +  f_{12}\\
     & = & 1/3 \times (\frac{f_{11}f_{22}}{f_{11}f_{22} + f_{12}f_{21}} + 1) \\
       &  & \hspace*{1cm} +
         1/3 \times (\frac{f_{12}f_{21}}{f_{11}f_{22} + f_{12}f_{21}} + 1)\\
%      & = & 1/3 \times (\frac{f_{11}f_{22} + f_{12}f_{21}}{f_{11}f_{22} + f_{12}f_{21}} + 2)\\
      & = & 1
  \end{eqnarray*}
\done
\fi

%In a similar manner, we derive $f_{21}$ and $f_{22}$ as follows.

%$$
%  f_{21} = 1/3 \times (\frac{f_{12}f_{21}}{f_{11}f_{22} + f_{12}f_{21}} + 0)
%$$
%and
%$$
%  f_{22} = 1/3 \times (\frac{f_{11}f_{22}}{f_{11}f_{22} + f_{12}f_{21}} + 2)
%$$

%Then, we obtain
%$$
%  3f_{21}f_{11}f_{22} + 3f_{12}f_{21}^2 - f_{12}f_{21} = 0
%$$
%and
%$$
%  3f_{11}f_{22}^2 + 3f_{12}f_{21}f_{22} - 3f_{11}f_{22} - 2f_{12}f_{21} = 0
%$$
%respectively.

%Let $g_{21} = 3f_{21}f_{11}f_{22} + 3f_{12}f_{21}^2 - f_{12}f_{21}$
%and $g_{22} =  3f_{11}f_{22}^2 + 3f_{12}f_{21}f_{22} - 3f_{11}f_{22} - 2f_{12}f_{21}$.


\if 0
\hrulefill

Jacobian matrix $J$ of partial derivatives is shown as follows.

$$
J = \left(
\begin{array}{c c c c}
  \frac{\partial g_{11}}{\partial f_{11}} & \frac{\partial g_{11}}{\partial f_{12}} & \frac{\partial g_{11}}{\partial f_{21}} & \frac{\partial g_{11}}{\partial f_{22}} \\
  \frac{\partial g_{12}}{\partial f_{11}} & \frac{\partial g_{12}}{\partial f_{12}} & \frac{\partial g_{12}}{\partial f_{21}} & \frac{\partial g_{12}}{\partial f_{22}} \\
  \frac{\partial g_{21}}{\partial f_{11}} & \frac{\partial g_{21}}{\partial f_{12}} & \frac{\partial g_{21}}{\partial f_{21}} & \frac{\partial g_{21}}{\partial f_{22}} \\
  \frac{\partial g_{22}}{\partial f_{11}} & \frac{\partial g_{22}}{\partial f_{12}} & \frac{\partial g_{22}}{\partial f_{21}} & \frac{\partial g_{22}}{\partial f_{22}}
\end{array}\right)
$$

\if 0
{\scriptsize
$$
\begin{array}{c c c c}
  6f_{11}f_{22} + 3f_{12}f_{21} - 2f_{22} & 3f_{11}f_{21} & 3f_{11}f_{12}-f_{12} & 3f_{11}^2-2f_{11} \\
  3f_{22}f_{12} & 3f_{11}f_{22} + 6f_{12}f_{21} - 2f_{21} & 3f_{12}^2 - 2f_{12} & 3f_{11}f_{12} - f_{11} \\
  3f_{21}f_{22} & 3f_{21}^2 - f_{21} & 3f_{11}f_{22} + 6f_{12}f_{21} - f_{12} & 3f_{21}f_{11} \\
  3f_{22}^2 - 3f_{22} & 3f_{21}f_{22} - 2f_{21} & 3f_{12}f_{22} - 2f_{12} & 6f_{11}f_{22}+3f_{12}f_{21}-3f_{11} \\
\end{array}
$$
}
\fi

where
{\scriptsize
\begin{eqnarray*}
  \frac{\partial g_{11}}{\partial f_{11}} = 6f_{11}f_{22} + 3f_{12}f_{21} - 2f_{22} &
  \frac{\partial g_{11}}{\partial f_{12}} = 3f_{11}f_{21}\\
  \frac{\partial g_{11}}{\partial f_{21}} = 3f_{11}f_{12}-f_{12} &
  \frac{\partial g_{11}}{\partial f_{22}} = 3f_{11}^2-2f_{11}\\
  \frac{\partial g_{12}}{\partial f_{11}} = 3f_{22}f_{12} &
  \frac{\partial g_{12}}{\partial f_{12}} = 3f_{11}f_{22} + 6f_{12}f_{21} - 2f_{21}\\
  \frac{\partial g_{12}}{\partial f_{21}} = 3f_{12}^2 - 2f_{12} &
  \frac{\partial g_{12}}{\partial f_{22}} = 3f_{11}f_{12} - f_{11}\\
  \frac{\partial g_{21}}{\partial f_{11}} = 3f_{21}f_{22} &
  \frac{\partial g_{21}}{\partial f_{12}} = 3f_{21}^2 - f_{21}\\
  \frac{\partial g_{21}}{\partial f_{21}} = 3f_{11}f_{22} + 6f_{12}f_{21} - f_{12} &
  \frac{\partial g_{21}}{\partial f_{22}} = 3f_{21}f_{11}\\
  \frac{\partial g_{22}}{\partial f_{11}} = 3f_{22}^2 - 3f_{22} &
  \frac{\partial g_{22}}{\partial f_{12}} = 3f_{21}f_{22} - 2f_{21}\\
  \frac{\partial g_{22}}{\partial f_{21}} = 3f_{12}f_{22} - 2f_{12} &
  \frac{\partial g_{22}}{\partial f_{22}} = 6f_{11}f_{22}+3f_{12}f_{21}-3f_{11}
\end{eqnarray*}
}

The values of $(f_{11}, f_{12}, f_{21}, f_{22})$ can be initialized to
any values such that
$$f_{11} + f_{12} = 1$$ and $$f_{21} + f_{22} = 1$$
But, for the sake of fast convergence, we can compute the initialization as follows.
$$
  f_{ij} = \frac{\sum_{L_k \in \mathcal{L}_{a_i}}c_k(a_i:x)}{\sum_{L_k \in \mathcal{L}_{a_i}} |L_k(a_i)|}
$$
where $c_k(a_i:x) = |L_k(a_i)| \times \frac{|L_k(x)|}{|L_k|}$
and $|L_k(x)|$ is the number of tuples in $L_k$ with sensitive value $x$.


By this initialization, the values $v=(f_{11}, f_{12}, f_{21}, f_{22})$ are initialized to $(1/2, 1/2, 1/6, 5/6)$.
By Newton's method, we adopt the formula
$$
  v_{n+1} = v_{n} - J^{-1} F_{n}
$$
where $v_{n}$ is a vector storing the values of $v$ at the $n$-th iteration
and $F_{n}$ is a vector storing the values of $(g_{11}, g_{12}, g_{21}, g_{22})$
at the $n$-th iteration.

The following shows the values of $v$ from the first iteration
to the 8-th iteration.

{\small
\begin{tabular}{| c | c| c| c| c|} \hline
Iteration & $f_{11}$ & $f_{12}$ & $f_{21}$ & $f_{22}$ \\ \hline
1 & 0.500000  &  0.500000    &  0.166667   &   0.833333 \\ \hline
2 & 0.833333   &   0.166667   &   -0.166667  &   1.166667 \\ \hline
3 & 0.717391   &   0.282609   &   -0.050725  &   1.050725 \\ \hline
4 & 0.673167   &   0.326833   &   -0.006500  &   1.006500 \\ \hline
5 & 0.666791  &    0.333209   &   -0.000124  &   1.000124 \\ \hline
6 & 0.666667   &   0.333333   &   0.000000   &   1.000000 \\ \hline
7 & 0.666667  &    0.333333   &   0.000000   &   1.000000 \\ \hline
8 & 0.666667   &   0.333333   &   0.000000  &    1.000000 \\ \hline
\end{tabular}
}

From the above iterations, we know that
$f_{11} = 0.666667, f_{12} = 0.333333, f_{21} = 0.000000$
and $f_{22} = 1.000000$.

Suppose we continue to compute $Pr(a_1:x_1|O)$ with
the above global distribution.
There is a privacy breach.
Consider the first equivalence class $L$.
There are two possible worlds, $\{a_1:x_1, a_2:x_2\}$
and $\{a_1:x_2, a_2:x_1\}$.
$P(a_1:x_1, a_2:x_2|G) =0.6667\times 1.0000 = 0.6667$
and $P(a_1:x_2, a_2:x_1|G) = 0.3333 \times 0.0000 = 0.0000$.
Thus, $P(a_1:x_1, a_2:x_2|O_1)=0.6667/(0.6667+0)=1$
and $P(a_1:x_2, a_2:x_1|O_1) = 0/(0.6667+0)=0$.
Thus, $Pr(a_1:x_1|O_1) = P(a_1:x_1, a_2:x_2|O_1) = 1$
which is greater than 1/2 (the objective of 2-diversity).


\subsubsection{Convergence and Uniqueness?}

%If the set of non-linear equations satisfies some conditions
%in contraction mapping
%theorem, we can achieve a unique solution with a convergence guarantee.
%The following shows the contraction mapping theorem.

\begin{theorem}
Let $R = I_1 \times I_2 \times ... \times I_n$ be a cartesian
product of closed intervals of finite length. Let $G(X)$ be a
function with domain $R$ and range contained in $R$.
\begin{itemize}
\item
If $G(X)$ is continuous, then $X=G(X)$ has at least one solution in
$R$.
\item
Suppose that there exists a constant $k < 1$ such that the row norm
or column norm of the Jacobian matrix of $G(X)$ does not exceed $k$,
for all $X \in R$. Then $X = G(X)$ has a unique solution $P \in R$,
and if $P_0 \in R$, $P_{m+1} = G(P_m)$, for $m = 0, 1, ...$, then
$\lim_{m \rightarrow \infty} P_m = P$.
\end{itemize}
\end{theorem}

%\begin{theorem}[Contraction Mapping Theorem]
%Suppose the set of $d$ equations on a solution space
%$x \in R^d$ are denoted by $g$.
%Suppose the set of equations $x = g(x)$ has a solution
%when $x = \alpha$.
%Let $B_a = \{x \in R^d |\ ||x - \alpha|| < a\}$ denote the open ball
%of radius $a$ centered on $\alpha$.
%If there is a constant $G < 1$ such that $\frac{||g(x) - g(y)||}{x - y} \le G$
%for all $x, y \in B_a$, then
%\begin{enumerate}
%  \item the set of equations $x = g(x)$ has exactly one solution over $B_a$, and
%  \item for any $x_0 \in B_a$, the sequence of iterates $x_0$, $g(x_0)$,
%  $g(g(x_0))$,... converges to the fixed point $\alpha$ of $g$.
%\end{enumerate}
%\label{th:contractionMappingThm}
%\end{theorem}

%We know that a solution $(f_{11}, f_{12}, f_{21}, f_{22}) =
%(0.666667, 0.333333, 0.000000, 1.000000)$.


Let us re-write the equations in the previous section in the following forms.

$$
f_{11}= \frac{1}{3} \times (\frac{f_{11}f_{22}}{f_{11}f_{22} + f_{12}f_{21}} + 1)
$$
$$
f_{12} = \frac{1}{3} \times (\frac{f_{12}f_{21}}{f_{11}f_{22} + f_{12}f_{21}} + 1)
$$
$$
f_{21} = \frac{1}{3} \times (\frac{f_{12}f_{21}}{f_{11}f_{22} + f_{12}f_{21}} + 0)
$$
$$
f_{22}= \frac{1}{3} \times (\frac{f_{11}f_{22}}{f_{11}f_{22} + f_{12}f_{21}} + 2)
$$

Let $h_1, h_2, h_3$ and $h_4$ be the right-hand-side of the above equations, respectively.
That is,
$$
h_1 = \frac{1}{3} \times (\frac{f_{11}f_{22}}{f_{11}f_{22} + f_{12}f_{21}} + 1)
$$
$$
h_2 = \frac{1}{3} \times (\frac{f_{12}f_{21}}{f_{11}f_{22} + f_{12}f_{21}} + 1)
$$
$$
h_3 = \frac{1}{3} \times (\frac{f_{12}f_{21}}{f_{11}f_{22} + f_{12}f_{21}} + 0)
$$
$$
h_4 = \frac{1}{3} \times (\frac{f_{11}f_{22}}{f_{11}f_{22} + f_{12}f_{21}} + 2)
$$

We obtain the following form.
$$
  x = g(x)
$$
where $x =
\left(
\begin{array}{c}
  f_{11} \\
  f_{12} \\
  f_{21} \\
  f_{22}
\end{array}
\right)$
and
$g(x) =
\left(
\begin{array}{c}
  h_1 \\
  h_2 \\
  h_3 \\
  h_4
\end{array}
\right)$

Now, we perform a partial derivative of $h_1$, $h_2$,
$h_3$ and $h_4$ with respect to $f_{11}$, $f_{12}$,
$f_{21}$ and $f_{22}$ as follows.

The partial derivatives of $h_1$ with respect
to $f_{11}$, $f_{12}$,
$f_{21}$ and $f_{22}$ are shown as follows.

$$
\frac{\partial h_1}{\partial f_{11}} = \frac{1}{3} \times \frac{f_{12}f_{21}f_{22}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_1}{\partial f_{12}} = \frac{1}{3} \times \frac{-f_{11}f_{22}f_{21}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_1}{\partial f_{12}} = \frac{1}{3} \times \frac{-f_{11}f_{22}f_{12}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_1}{\partial f_{22}} = \frac{1}{3} \times \frac{f_{11}f_{12}f_{21}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$

%\hrulefill

The partial derivatives of $h_2$ with respect
to $f_{11}$, $f_{12}$,
$f_{21}$ and $f_{22}$ are shown as follows.

$$
\frac{\partial h_2}{\partial f_{11}} = \frac{1}{3} \times \frac{-f_{12}f_{21}f_{22}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_2}{\partial f_{12}} = \frac{1}{3} \times \frac{f_{11}f_{22}f_{21}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_2}{\partial f_{12}} = \frac{1}{3} \times \frac{f_{11}f_{22}f_{12}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_2}{\partial f_{22}} = \frac{1}{3} \times \frac{-f_{12}f_{21}f_{11}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$

%\hrulefill

The partial derivatives of $h_3$ with respect
to $f_{11}$, $f_{12}$,
$f_{21}$ and $f_{22}$ are shown as follows.

$$
\frac{\partial h_3}{\partial f_{11}} = \frac{1}{3} \times \frac{-f_{12}f_{21}f_{22}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_3}{\partial f_{12}} = \frac{1}{3} \times \frac{f_{11}f_{22}f_{21}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_3}{\partial f_{12}} = \frac{1}{3} \times \frac{f_{11}f_{22}f_{12}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_3}{\partial f_{22}} = \frac{1}{3} \times \frac{-f_{12}f_{21}f_{11}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$

%\hrulefill

The partial derivatives of $h_4$ with respect
to $f_{11}$, $f_{12}$,
$f_{21}$ and $f_{22}$ are shown as follows.

$$
\frac{\partial h_4}{\partial f_{11}} = \frac{1}{3} \times \frac{f_{12}f_{21}f_{22}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_4}{\partial f_{12}} = \frac{1}{3} \times \frac{-f_{11}f_{22}f_{21}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_4}{\partial f_{12}} = \frac{1}{3} \times \frac{-f_{11}f_{22}f_{12}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$
$$
\frac{\partial h_4}{\partial f_{22}} = \frac{1}{3} \times \frac{f_{11}f_{12}f_{21}}{(f_{11}f_{22} + f_{12}f_{21})^2}
$$

Let $\triangle = (\sum_{k=1,2,3,4}\sum_{i = 1, 2}\sum_{j = 1, 2}(\frac{\partial h_k}{\partial f_{ij}})^2)^{1/2}$.
If we show that $\triangle < 1$,
then
 $\frac{||g(x) - g(y)||}{x - y} \le G$ where $G < 1$.
By Theorem~\ref{th:contractionMappingThm}, we know
that $x = g(x)$ has a unique solution.

In the following, we evaluate $\triangle$
of each iteration (computed previously).

\noindent
{\scriptsize
\begin{tabular}{| c | c | c | c | c | c |} \hline
Iteration & $f_{11}$ & $f_{12}$ & $f_{21}$ & $f_{22}$ & $\triangle$ \\ \hline
1 & 0.500000  &  0.500000   &   0.167000  &    0.833000  &    0.624159 \\ \hline
2 & 0.833333  &    0.166667  &    -0.166667  &   1.166667   &   0.173839 \\ \hline
3 & 0.717391  &    0.282609  &    -0.050725  &   1.050725   &   0.264819 \\ \hline
4 & 0.673167  &    0.326833  &    -0.006500  &   1.006500   &   0.323699 \\ \hline
5 & 0.666791  &    0.333209  &    -0.000124  &   1.000124   &   0.333148 \\ \hline
6 & 0.666667  &    0.333333  &    0.000000   &   1.000000  &    0.333333 \\ \hline
7 & 0.666667  &    0.333333  &    0.000000   &   1.000000   &   0.333333 \\ \hline
8 & 0.666667  &    0.333333  &    0.000000  &    1.000000  &    0.333333 \\ \hline
\end{tabular}
}

From the above iterations, we know that, during the iterative
process, $\triangle$ is always smaller than 1.
Then, $x = g(x)$ has a unique solution and the iterative
process converges to this unique solution.

From \cite{PC88}, ``we can assert that it will converge provided the
initial approximation is `sufficiently close' to the solution which
is sought; the assertion stems from the use of the generalized
contraction mapping theorem."

With this assertion, if we choose an initial approximation
close to the solution, then it will converge.
Thus, our initial approximation for the probability $f_{ij}$ that $a_i$ is linked to $x$
is also estimated by evaluating
the sum of
the proportions of $x$ in all equivalence classes $L$ containing $a_i$.
That is,
$$
  f_{ij} = \frac{\sum_{L_k \in \mathcal{L}_{a_i}}c_k(a_i:x)}{\sum_{L_k \in \mathcal{L}_{a_i}} |L_k(a_i)|}
$$
where $c_k(a_i:x) = |L_k(a_i)| \times \frac{|L_k(x)|}{|L_k|}$
and $|L_k(x)|$ is the number of tuples in $L_k$ with sensitive value $x$.

It is noted that some solutions do not give $
\triangle < 1$. For example,
if $(f_{11}, f_{12}, f_{21}, f_{22}) =
(0, 1, 0.1, 0.9), \triangle = 6 > 1$.
If $(f_{11}, f_{12}, f_{21}, f_{22}) =
(0.9, 0.1, 0.9, 0.1), \triangle = 2.371527 > 1$.
But, these solutions are not close
to the unique solution.)

\fi

%

